HelpBench: Assessing the Ability of LLMs to Provide Privacy, Safety, and Security Advice

This paper introduces HelpBench, a benchmark for assessing whether LLMs are capable of providing accurate help in response to questions about digital privacy, safety, and security. We curated 450 questions representing authentic user situations and developed rubrics for each question to evaluate the factual accuracy and tone of a response. Example questions touch on how to regain access to lost or suspended accounts, how to balance the trade-offs of hardware security keys versus other forms of two-factor authentication, whether a suspicious email is likely a scam, or whether an abuser might be able to track an individual based on their device peripherals. We then developed and applied an auto-rater to evaluate responses from 18 state-of-the-art LLMs. Our results indicate that while models provide high-quality advice (with scores of 82% on average), one in ten responses from models scores less than 65%, reflecting inaccurate and even harmful advice. Addressing these failures is critical for models to serve as trustworthy sources of assistance for digital privacy, safety, and security needs.

==> F_stats.tex <==

\section{Details on Statistical Analysis}
\label{app:stats}

To account for likely clustering in the scores for responses to the same question, we run statistical tests using permutation tests rather than applying a test directly; e.g., we use a permutation test with the Kruskal-Wallis statistic rather than applying the Kruskal-Wallis test to all model responses. For the sake of reproducibility, we provide details and code for this approach here.



==> Makefile <==
all: main.pdf

main.pdf:  *.tex *.bib
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main
	pdflatex main

clean:
	rm -f *.bak
	rm -f *~
	rm -f main.pdf
	rm -f main.ps
	rm -f *.log
	rm -f *.aux*
	rm -f *.dvi
	rm -f *.bbl
	rm -f *.blg
	rm -f *.idx
	rm -f *.out

rubber:
	rubber --pdf -Wall --warn misc main.tex
	rubber-info main.tex

watch:
	make rubber
	- while true; do \
	  	inotifywait -r -e DELETE_SELF -e MOVE_SELF -e MODIFY *.tex *.bib tables/*.tex figs/*; \
			make rubber; \
			sleep 1; \
		done

